SmartPQ: An Adaptive Concurrent Priority Queue for NUMA Architectures

Concurrent priority queues are widely used in important workloads, such as graph applications and discrete event simulations. However, designing scalable concurrent priority queues for NUMA architectures is challenging. Even though several NUMA-oblivious implementations can scale up to a high number of threads, exploiting the potential parallelism of insert operation, NUMA-oblivious implementations scale poorly in deleteMin-dominated workloads. This is because all threads compete for accessing the same memory locations, i.e., the highest-priority element of the queue, thus incurring excessive cache coherence traffic and non-uniform memory accesses between nodes of a NUMA system. In such scenarios, NUMA-aware implementations are typically used to improve system performance on a NUMA system. In this work, we propose an adaptive priority queue, called SmartPQ. SmartPQ tunes itself by switching between a NUMA-oblivious and a NUMA-aware algorithmic mode to achieve high performance under all various contention scenarios. SmartPQ has two key components. First, it is built on top of NUMA Node Delegation (Nuddle), a generic low-overhead technique to construct efficient NUMA-aware data structures using any arbitrary concurrent NUMA-oblivious implementation as its backbone. Second, SmartPQ integrates a lightweight decision making mechanism to decide when to switch between NUMA-oblivious and NUMA-aware algorithmic modes. Our evaluation shows that, in NUMA systems, SmartPQ performs best in all various contention scenarios with 87.9% success rate, and dynamically adapts between NUMA-aware and NUMA-oblivious algorithmic mode, with negligible performance overheads. SmartPQ improves performance by 1.87x on average over SprayList, the state-of-theart NUMA-oblivious priority queue.

==> 3_classifier.tex <==

\section{Selecting \arxiv{t}he \arxiv{A}lgorithmic Mode}

As already discussed, \arxiv{the performance of a priority queue implementation is becoming increasingly dependent on both the contention levels of the workload and the underlying computing platform.} In this section, we propose a decision making mechanism\arxiv{, which is based on machine learning, to select} the best-performing \algomode{} mode, \arxiv{i.e., between the \notnuma{} and \numa{} mode, for each contention workload in a NUMA system.}




\begin{figure*}
%\centering
    \centering\captionsetup[subfloat]{labelfont=bf}
  \begin{subfigure}[h]{0.48\textwidth}
    \centering
    \includegraphics[scale=0.154]{classifier/class_threads.pdf}
    \vspace{-1pt}
    \caption{} 
    %\label{fig:coherence} 
 \end{subfigure}
  ~
  \begin{subfigure}[h]{0.48\textwidth}
   \centering
    \includegraphics[scale=0.154]{classifier/class_range.pdf}
    \vspace{-1pt}
    \caption{}
    %\label{fig:numaness}
  \end{subfigure} 
  %\vspace{-6pt}
  \caption{\arxiv{Throughput achieved by} \nuddle{} \arxiv{(using 8 server threads)} and its underlying \notnuma{} \arxiv{\emph{base algorithm}, \arxiv{i.e., alistarh\_herlihy~\cite{spraylist,herlihy},} as we vary} (a) the number of threads, and (b) the key range \arxiv{of the workload.}}
  \label{fig:nuddle_spraylist}
  \vspace{-6pt}
\end{figure*}


\subsection{The Need for \arxiv{a} Machine Learning \arxiv{Approach}}

Selecting \arxiv{the best-performing algorithmic mode can be solved in various ways. For instance, one could take an empirical \arxiv{exhaustive} approach: measure the throughput achieved by the two algorithmic modes for each particular contention workload on the target NUMA system, and then use the \algomode{} mode that achieves the highest throughput on future runs of the same contention workload on the target NUMA system. Even though this is the most accurate method, it (i) incurs \emph{substantial} overhead and effort to sweep over \emph{all} various contention workloads, and (ii) would need a large amount of memory to keep the best-performing \algomode{} mode for the various contention workloads on each NUMA system. Furthermore, it is not trivial to construct a statistical model to predict the best-performing \algomode{} mode, since the performance is also affected by the characteristics of underlying computing platform. Figure~\ref{fig:nuddle_spraylist} summarizes these observations, comparing \nuddle{} (\numa{}) with its underlying \notnuma{} \emph{base algorithm}, i.e., alistarh\_herlihy~\cite{spraylist,herlihy}. We \arxiv{use} a 4-socket NUMA server, which is described in \arxiv{S}ection \ref{sec:experimental}.}



Figure~\ref{fig:nuddle_spraylist}a \arxiv{demonstrates that the best-performing \algomode{} mode depends on various parameters, including the number of running threads, the size of the data structure, and the operation workload, i.e., the \arxiv{percentage} of \insrt/\delete{} operations. Specifically,} when the number of \arxiv{running} threads increases, the contention also increases, and thus we may expect that the performance of \arxiv{the \notnuma{}} alistarh\_herlihy degrades. \arxiv{In contrast,} when using 29 threads with 80\% \insrt{} operations, alistarh\_herlihy outperforms \nuddle. \arxiv{This is because} the size of the priority queue and the key range \arxiv{of the workload} are relatively large, \arxiv{and at the same time} the \arxiv{percentage} of \delete{} operations is \arxiv{low.} \arxiv{In this scenario}, threads \arxiv{may work
on different elements of the data structure,} and thus, \arxiv{the \notnuma{}} alistarh\_herlihy achieves high throughput.


Figure~\ref{fig:nuddle_spraylist}b \arxiv{shows that the best-performing \algomode{} mode cannot be straightforwardly predicted, and also depends on the key range of the workload and the characteristics of underlying hardware.} In \insrt-dominated workloads, as the key range increases, the contention decreases, since threads compete less for the same elements. We might, thus, expect that after a certain point, \arxiv{the \notnuma{}} alistarh\_herlihy will always outperform \nuddle, \arxiv{since} the contention decreases. However, when using \arxiv{50 running threads and} the key range of 10K, alistarh\_herlihy achieves 1.58$\times$ performance \arxiv{slowdown over} \nuddle{}. In this \arxiv{experiment, we note that, even though} the performance of \nuddle{} remains constant, as expected, the performance of alistarh\_herlihy varies as the key range changes, due to the hyperthreading effect. When using more than 32 threads, hyperthreading is enabled in our NUMA server resulting to a varying behavior \arxiv{for} alistarh\_herlihy \arxiv{implementation.} The hyperthreading pair of threads shares the L1 and L2 caches\arxiv{, and thus, these threads} may either thrash or benefit from each other depending on \arxiv{the characteristics of L1 and L2 caches (e.g., size, eviction policy), and} the elements accessed in each operation.

Consequently, considering \arxiv{the above observations and the high overhead of an exhaustive approach,} we resort to \arxiv{a} machine learning \arxiv{approach} as the basis of \arxiv{our} prediction mechanism for \arxiv{the aforementioned} non-straightforward behavior. 



\subsection{Decision Tree Classifier}\label{sec:classifier}
We formulate the selection of the \algomode{} mode as a classification problem, and leverage supervised learning techniques to train a classifier \arxiv{which can be used to predict} the \arxiv{best-performing} \algomode{} mode for each \arxiv{contention} workload. For our classifier, we \arxiv{select} decision trees, since they are commonly used \arxiv{in} classification models~\cite{athena}\cgiannou{Add more references}, \arxiv{and incur} low training and inference \arxiv{overhead}. Moreover, they are easy to interpret and thus, be incorporated to \arxiv{our} proposed priority queue (Section~\ref{SmartPQbl}). We generate the decision tree classifier using the scikit-learn machine learning toolkit~\cite{scikit}. 



\textbf{\textit{1) Class Definition:}} 
\arxiv{We define the following classes:} (a) the \textbf{\notnuma} class that stands for the \notnuma{} \algomode{} mode, (b) the \textbf{\numa{}} class that stands for the \numa{} \algomode{} mode, and (c) the \textbf{\textit{neutral}} class that stands for "tie", meaning that \arxiv{either a \numa{} or a \notnuma{} implementation can be selected, since they achieve similar performance. We include a neutral class for two reasons:} (i) when using \emph{only one} socket of \arxiv{a NUMA system}, \numa{} implementations deliver \arxiv{similar throughput with \notnuma{} implementations, and (ii) in an adaptive data structure, i.e., which \emph{dynamically} switches between the two \algomode{} modes,} we want to configure a transition from one \arxiv{\algomode{} mode} to another to occur when the difference in their throughput is \arxiv{relatively high, i.e.,} greater than a certain threshold. Otherwise, \arxiv{the adaptive data structure} might continuously oscillate between the two modes, without delivering significant performance improvement or even causing performance degradation.


 
\textbf{\textit{2) \arxiv{Extracted Features}}}: \arxiv{Table~\ref{table:features} shows the 4 features used in our proposed classifier, which targets priority queues. We assume that the contention workload is known a priori, and thus, we can easily extract the features needed for classification. Section~\ref{sec:discussion} discusses how to on-the-fly extract these features.} 



\begin{table}[H]
\centering
%\ra{0.9}
\resizebox{\linewidth}{!}{
\begin{tabular}{l l} 
 \toprule
 Feature & Definition  \\ [0.5ex] \midrule \midrule
% \hline\hline
 \#threads & The number of running threads \\
 size & The \arxiv{current} size of the priority queue\\
% key\_range & The range of keys used in requested \\
% & operations\\
key\_range & The range of keys used in operations \\
 \% \insrt /\delete & The \arxiv{percentage} of \insrt /\delete{} operations\\
 \bottomrule
\end{tabular}
}
\caption{The features used for classification.}
\label{table:features}
\end{table}


==> 4a_smartPQ.tex <==

\section{\smartpq} \label{SmartPQbl}

We propose \arxiv{\smartpq, an adaptive priority queue which \emph{dynamically} switches between \notnuma{} and \numa{} \algomode{} modes, to achieve the highest available performance at \emph{any} point in time, even when the contention of the workload varies over time.}

Designing an adaptive priority queue, \arxiv{which switches between two \algomode{} modes, involves addressing two challenges: (i)} how to switch \arxiv{between the \algomode{} modes} with \emph{low overhead}, and \arxiv{(ii) \emph{when} to switch from one \algomode{} mode to the other. 

To address the first challenge, we exploit the fact that the actual underlying implementation of \nuddle{} is a \emph{concurrent} \notnuma{} implementation. We select \nuddle{}, as the \numa{} \algomode{} mode of \smartpq{}, and its underlying \emph{base algorithm}, as the \notnuma{} \algomode{} mode of \smartpq. Threads can perform operations in the data structure using either \nuddle{} or its underlying \emph{base algorithm}, with no actual change in the way data is accessed. As a result, \smartpq{} can switch between the two \algomode{} modes without needing a synchronization point between transitions, i.e., with negligible  performance overheads, and without violating correctness.

To address the second challenge, we (i) train the proposed classifier (Section~\ref{sec:classifier}) using \nuddle{}, as the \numa{} implementation, and its underlying \emph{base algorithm}, as the \notnuma{} implementation, and (ii) incorporate a \emph{lightweight} decision making mechanism in \smartpq{} to predict \emph{when} a transition to another \algomode{} mode is needed. We describe the details in the next section.
} 

\subsection{Implementation Details}

\textbf{\textit{Generation of Training Data:}}
To train our classifier, we develop microbenchmarks in which threads execute random operations on the \arxiv{priority queue} for 5 seconds. We \arxiv{select} \nuddle{}, as the \numa{} \arxiv{implementation}, and \emph{alistarh\_herlihy}, as \arxiv{its underlying} \notnuma{} \arxiv{implementation, since this is the \notnuma{} priority queue that achieves the highest throughput according to our evaluation (Section~\ref{sec:experimental}). We use} a variety of values for the features \arxiv{needed for classification} (Table~\ref{table:features}). Our training data set consists of 5525 different \arxiv{contention} workloads. Finally, \arxiv{note that} we pin software threads to hardware threads \arxiv{in the evaluated NUMA system} in a round-robin fashion, and thus, the classifier is trained \arxiv{with} this thread placement. \arxiv{We leave the exploration of the thread placement policy for future work.}
 


\textbf{\textit{Labeling of Training Data:}}
Regarding \arxiv{the labeling of our training} data set, we set the threshold for "tie" between the two \algomode{} modes to \arxiv{an empirical value, i.e.,} 1.5 Million operations per second. When the difference in throughput \arxiv{between the two \algomode{} modes} is less than this threshold, the \textit{neutral} class is selected as label. Otherwise, we select the class that corresponds to the \algomode{} mode that \arxiv{achieves} the higher throughput.

The final decision tree classifier has \arxiv{only} 180 nodes, half of which are leaves. It has a quite low depth of 8, that is the length of the longest path in the tree, and consequently, a quite \emph{low} traversal cost (2-4 ms in \arxiv{our evaluated NUMA system).} 

%we call the classifier in a fixed time interval of 1 second. Every second, a thread calls the classifier to detect if a transition to another mode is needed. If this is the case, the algo variable is updated and SmartPQ switches mode
 


Figure~\ref{alg:smartpq} presents the modified code of \nuddle{} \arxiv{adding the decision making mechanism} to implement \smartpq.
We extend the main structure of \nuddle{}, renamed to {\fontfamily{lmtt}\selectfont \textit{struct smartpq}}, by adding an additional field, named {\fontfamily{lmtt}\selectfont \textit{algo}}, \arxiv{to keep} track the current \algomode{} mode, i.e., either \nuddle{} or \arxiv{its \emph{base algorithm}}. Similarly, {\fontfamily{lmtt}\selectfont \textit{struct client}} and {\fontfamily{lmtt}\selectfont \textit{struct server}} \arxiv{structures} are extended with an additional {\fontfamily{lmtt}\selectfont \textit{algo}} field, \arxiv{which} is a pointer to the {\fontfamily{lmtt}\selectfont \textit{algo}} \arxiv{field of the main structure, i.e., {\fontfamily{lmtt}\selectfont \textit{struct smartpq}}.} \arxiv{Each running thread initializes this pointer either} in {\fontfamily{lmtt}\selectfont \textit{initClient()}} \arxiv{or} {\fontfamily{lmtt}\selectfont \textit{initServer()}} depending on its role (e.g., line 119 in Fig.~\ref{alg:smartpq}). \arxiv{This} way, all threads share the same \algomode{} mode at any point in time. We also modify the core \arxiv{functions} of client \arxiv{threads, i.e., {\fontfamily{lmtt}\selectfont \textit{insert\_client()}} and {\fontfamily{lmtt}\selectfont \textit{deleteMin\_client()}}}, such that \arxiv{client threads} either directly execute their \arxiv{operations} in the data structure (e.g., line 126 in Fig.~\ref{alg:smartpq}), or delegate them to server \arxiv{threads} (e.g., line 128 in Fig.~\ref{alg:smartpq}), with respect to the current \algomode{} mode. \arxiv{In contrast}, the core \arxiv{functions} of server \arxiv{threads} do not need any modification. Finally, we wrap the lines \arxiv{79-90} of {\fontfamily{lmtt}\selectfont \textit{serve\_requests}} function of Figure~\ref{alg:functions} with an if/else statement on the {\fontfamily{lmtt}\selectfont \textit{algo}} field, such that server \arxiv{threads} poll at client \arxiv{threads}' requests only in \numa{} mode. \arxiv{In} \notnuma{} mode, {\fontfamily{lmtt}\selectfont \textit{serve\_requests}} function returns without doing \arxiv{nothing}. \arxiv{This} way, programmers do not need to take care of calls on this function in their code, when the \notnuma{} mode is selected.

\arxiv{The} {\fontfamily{lmtt}\selectfont \textit{decisionTree()}} \arxiv{function} describes the \arxiv{interface for our proposed decision tree} classifier, where the \arxiv{input} arguments are associated with its features. In frequent time lapses, one or more threads \arxiv{may} call this function to check if a transition to another \arxiv{\algomode{}} mode is needed. If this is the case, the {\fontfamily{lmtt}\selectfont \textit{algo}} field of {\fontfamily{lmtt}\selectfont \textit{struct smartpq}} is updated \arxiv{(line 154 in Fig.~\ref{alg:smartpq})}, \arxiv{and} \smartpq{} switches mode, \arxiv{i.e.,} all \arxiv{running} threads start executing their operations using the new \algomode{} mode. If the classifier predicts the neutral class \arxiv{(line 153 in Fig.~\ref{alg:smartpq})}, the {\fontfamily{lmtt}\selectfont \textit{algo}} field is not updated, and \arxiv{thus} \smartpq{} remains at the \arxiv{currently} selected \arxiv{\algomode{}} mode.



\begin{figure}[H]
\begin{lstlisting}[language=C]
struct smartpq {              
  (*\textcolor{darkred}{nm\_oblv\_set}*) *base_pq;      
  int servers, groups, clnt_per_group; 
  int server_cnt, clients_cnt, group_cnt;   
  cache_line *requests[groups][clnt_per_group]; 
  cache_line *responses[groups];     
  lock *global_lock;    
  (*\textcolor{darkgreen}{int *algo;}*) (*\textcolor{darkgreen}{// 1: NUMA-oblivious (default), \\ 2: NUMA-aware}*)
};

struct client {
  (*\textcolor{darkred}{nm\_oblv\_set}*) *base_pq;      
  cache_line *request, *response;   
  int clnt_pos;             
  (*\textcolor{darkgreen}{int *algo;}*)  
};

struct client *initClient(struct smartpq *pq) { 
  ... lines 60-69 of Fig. 5 ...
  cl->base_pq = pq->base_pq;
  (*\textcolor{darkgreen}{cl->algo = \&(pq->algo);}*)
  release_lock(pq->global_lock);  
  return cl; 
}

int insert_client(struct client *cl,                                   int key, float value) {
  (*\textcolor{darkgreen}{if( *(cl->algo) == 1) \{ }*)       
    return (*\textcolor{darkred}{\_\_base\_insert(cl->base\_pq,key,value);}*)
  (*\textcolor{darkgreen}{\} else \{ // *(cl->algo) == 2}*)
    ... lines 95-97 of Fig. 6 ...
  (*\textcolor{darkgreen}{\}}*)                         
}   

void serve_requests(struct server *srv) {
  (*\textcolor{darkgreen}{if( *(srv->algo) == 2)\{}*) 
    for(i = 0; i < srv->mygroups; i++) {
      cache_line resp;
      for(j = 0; j < srv->clnt_per_group; j++) {
        key = srv->my_clients[i][j].key;
        value = srv->my_clients[i][j].value;
        if (srv->my_clients[i][j].op == "insert")
          resp[j] = (*\textcolor{darkred}{\_\_base\_insrt}*)(srv->base_pq, key, value);  
        else if (srv->my_clients[i][j].op == "deleteMin")
          resp[j] = (*\textcolor{darkred}{\_\_base\_delMin}*)(srv->base_pq);
      }
      srv->my_responses[i] = resp;
    }
  (*\textcolor{darkgreen}{\} else}*)
    (*\textcolor{darkgreen}{return;}*)
}

void decisionTree(struct server/struct client *str,                    int nthreads, int size, (* \\ *) int key_range, double insert) {
  int algo = 0;
  ... code (*for*) decision tree classifier ...
  if (algo != 0) //  (*\textcolor{darkgreen}{0: neutral}*)  
    *(str->algo) = algo;
}
\end{lstlisting}
\caption{The modified code of \nuddle{} \arxiv{adding the decision making mechanism} to implement \smartpq{}.}
\label{alg:smartpq}
\end{figure}

